Intermediate Service Facility Planning in a Stochastic and Competitive Market: Incorporating Agent-infrastructure Interactions over Networks

This paper presents a network-based multi-agent optimization model for the strategic planning of service facilities in a stochastic and competitive market. We focus on the type of service facilities that are of intermediate nature, i.e., users may need to deviate from the shortest path to receive/provide services in between the users' planned origins and destinations. This problem has many applications in emerging transportation mobility, including dynamic ride-sharing hub design and competitive facility location and allocation problems for alternative fuel vehicle refueling stations. The main contribution of this paper is establishing a new multi-agent optimization framework considering decentralized decision makings of facility investors and users over a transportation network and providing rigorous analyses of its mathematical properties, such as uniqueness and existence of system equilibrium. In addition, we develop an exact convex reformulation of the original multi-agent optimization problems to overcome computational challenges brought by non-convexity. Extensive analysis on case studies showed how the proposed model can capture the complex interaction between different stakeholders in an uncertain environment. Additionally, our model allowed quantifying the value of stochastic modeling and information availability by exploring stochastic metrics, including value of stochastic solution (VSS) and expected value of perfect information (EVPI), in a multi-agent framework.

==> Appendices/app_derivatives.tex <==
% jd 2015-05-22 23:30
\chapter{Calculation of ${\partial \rho_{k'}}/{\partial g_i^j}$}\label{app: part_rho_part_g}

${\partial \rho_{k'}}/{\partial g_i^j}$ can be computed from the ISO's optimization problem (\ref{DP_ISO_nn_t}), where $\boldsymbol{\rho}$ is the dual variables of constraint (\ref{DP_ISO_fc2}) and $\boldsymbol{g}$ is parameters. ${\partial \rho_{k'}}/{\partial g_i^j}$ is essentially the derivative of dual variables with respect to right-hand side constants. We use the standard  notations for convex optimization with linear constraints:

\begin{subequations}\label{eq:stan_opti_nota}
\begin{alignat}{2}
\min_{\boldsymbol{x}}
&\phantom{===} \hspace{0.5cm} &&\phantom{=}f(\boldsymbol{x})   \label{stan_opti_of}\\
 \text{s.t.}
&\phantom{===} (\boldsymbol{\lambda}) &&\phantom{=}A\boldsymbol{x}=\boldsymbol{b}\label{stan_opti_cons}
\end{alignat}
\end{subequations}
 
\noindent where $f(\boldsymbol{x})$ is a convex function and $\boldsymbol{x} \in \mathbb{R}^n, \boldsymbol{\lambda}, \boldsymbol{b} \in \mathbb{R}^m$, to illustrate the calculating process and our goal is to calculate the Jacobian matrix $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$.

Lagrangian of problem (\ref{eq:stan_opti_nota}) is $\mathcal{L} = f(\boldsymbol{x}) - \boldsymbol{\lambda}^{T}(A\boldsymbol{x}-\boldsymbol{b})$. The optimality conditions of problem (\ref{eq:stan_opti_nota}) is:

\begin{subequations}\label{eq:stan_opti_opti_cond}
\begin{align}
\nabla f(\boldsymbol{x}) - A^T\boldsymbol{\lambda} &= \boldsymbol{0}\label{stan_opti_opti_cond1}\\
A\boldsymbol{x}-\boldsymbol{b} &= \boldsymbol{0}\label{stan_opti_opti_cond2}
\end{align}
\end{subequations}

Take implicit derivatives of equations (\ref{eq:stan_opti_opti_cond}) with respect to $\boldsymbol{b}$ :

\begin{subequations}\label{eq:stan_opti_opti_cond_impl_deri}
\begin{align}
\nabla^2_{\boldsymbol{x}} f(\boldsymbol{x^{\ast}}(\boldsymbol{b})) J_{\boldsymbol{x}}(\boldsymbol{b}) - A^T J_{\boldsymbol{\lambda}}(\boldsymbol{b}) &= \boldsymbol{0}\label{stan_opti_opti_cond1_impl_deri}\\
AJ_{\boldsymbol{x}}(\boldsymbol{b})-\boldsymbol{I} &= \boldsymbol{0}\label{stan_opti_opti_cond2_impl_deri}
\end{align}
\end{subequations}

The unknown variables in equations (\ref{eq:stan_opti_opti_cond_impl_deri}) are two Jacobian matrices, $J_{\boldsymbol{x}}(\boldsymbol{b})$ and $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$. The total number of equations is equal to the total number of variables in equations (\ref{eq:stan_opti_opti_cond_impl_deri}), which is $nm+m^2$. Therefore, in most cases, $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$ can be calculated given $\boldsymbol{b}$. Numerically, one can take an initial guess of $\boldsymbol{b}$ based on historical data and then solve equations (\ref{eq:stan_opti_opti_cond_impl_deri}) and Algorithm \ref{alg: ph_trans} iteratively until $J_{\boldsymbol{\lambda}}(\boldsymbol{b})$ converged.






==> Appendices/app_flow.tex <==
\chapter{Small Example Illustrating Flow Conservation Constraint (\ref{DP_ISO_alf}) $\sim$ (\ref{DP_ISO_fc3})}\label{App:flow_exam}

\subsection*{Network Structure}
 \begin{figure}[htbp]
\begin{center}
    \includegraphics[width=0.4\textwidth]{./Figures/Energy/6node_network_structure.pdf}
\caption{Small Example Structure}
\label{fig:smal_exam_stru}
\end{center}
\end{figure}

\subsection*{OD and Path Information}
 \begin{table}[htbp]
 \caption{Small Example Structure}
 \vspace{-0.5cm}
\begin{center}
    \includegraphics[width=0.7\textwidth]{./Figures/Energy/od_path.pdf}
\label{fig:od_path}
\end{center}
\end{table}
\pagebreak
\subsection*{Network Flow}
 \begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\textwidth]{./Figures/Energy/network_flow.pdf}
\label{fig:netw_flow}
\caption*{}
\end{center}
\end{figure}
\vspace{-2cm}
\subsection*{Incidence Matrix}
 \begin{figure}[h]
\begin{center}
    \includegraphics[width=0.9\textwidth]{./Figures/Energy/incidence_matrix.pdf}
\label{fig:inci_matr}
\caption*{}
\end{center}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
